A general approach for identifying hierarchical symmetry constraints for analog circuit layout

Analog layout synthesis requires some elements in the circuit netlist to be matched and placed symmetrically. However, the set of symmetries is very circuit-specific and a versatile algorithm, applicable to a broad variety of circuits, has been elusive. This paper presents a general methodology for the automated generation of symmetry constraints, and applies these constraints to guide automated layout synthesis. While prior approaches were restricted to identifying simple symmetries, the proposed method operates hierarchically and uses graph-based algorithms to extract multiple axes of symmetry within a circuit. An important ingredient of the algorithm is its ability to identify arrays of repeated structures. In some circuits, the repeated structures are not perfect replicas and can only be found through approximate graph matching. A fast graph neural network based methodology is developed for this purpose, based on evaluating the graph edit distance. The utility of this algorithm is demonstrated on a variety of circuits, including operational amplifiers, data converters, equalizers, and low-noise amplifiers.

==> misc/customize-old.tex <==
% ADDED BY VIVEK
%\usepackage[latin1]{inputenc}
\usepackage{amsmath}
\usepackage{hhline}
\usepackage{silence}
\usepackage{graphicx}
\usepackage{multirow} 
\usepackage{graphicx}
\usepackage{multirow}
\usepackage{amsmath}
\usepackage[english]{babel}
\usepackage{booktabs}
\usepackage{array}
\usepackage{paralist}
\usepackage{threeparttable}
\usepackage{lipsum}
\usepackage{flushend}
\usepackage{cuted}
% not available \usepackage{algpseudocode}
\usepackage{algorithm2e}
% not available  \usepackage{algcompatible}
%\usepackage{acmcopyright}
\usepackage{amssymb}
\usepackage{color}
\usepackage{psfrag}
\usepackage{epsfig}
\usepackage{multicol}
\usepackage{color}
\usepackage{fancybox}
\usepackage{subfigure}
\usepackage{cite}
\usepackage{theorem}
\usepackage{url}
\usepackage[table]{xcolor}
\usepackage{epstopdf}
\usepackage[normalem]{ulem}
%not available \usepackage{siunitx}
%\usepackage{subcaption}
\usepackage[justification=centering,font=small,labelfont=bf]{caption}
\usepackage{silence}
\WarningFilter{caption}{Unsupported document class}
\usepackage{enumitem}
%\usepackage{widetext}
%\usepackage{paralist}
%\usepackage[none]{hyphenat}
\hyphenation{intersection op-tical net-works semi-conductor Electro-migration immortality}
\definecolor{gray1}{gray}{0.90}
\definecolor{gray2}{gray}{0.98}
\definecolor{light-gray}{gray}{0.95}
\def\bibfont{\scriptsize}
%Adds extra padding to the table cells
\setlength\extrarowheight{2pt}

\newcommand{\ignore}[1]{}
\newcommand{\redHL}[1]{\textcolor{red}{#1}}
\newcommand{\blueHL}[1]{{\textcolor{blue}{#1}}}
\newcommand{\greenHL}[1]{\textcolor{green}{#1}}
\newcommand{\blackHL}[1]{\textcolor{black}{#1}}
\newcommand{\Alter}[2]{\sout{#1}\redHL{#2}}
\newcommand{\Deff}{D_{\mbox{\tiny \em eff}}}
\newcommand{\Deffn}{D_{\mbox{\tiny \em eff,n}}}
\newcommand{\Deffg}{D_{\mbox{\tiny \em eff,g}}}
\newcommand{\Zeff}{Z^\star_{\mbox{\tiny \em eff}}}
\newcommand{\Javg}{J_{\mbox{\tiny \em avg}}}
\newcommand{\Jeff}{J_{\mbox{\tiny \em eff}}}
\newcommand{\Jrms}{J_{\mbox{\tiny \em rms}}}
\newcommand{\Jflux}{J_{\mbox{\tiny \em flux}}}
\newcommand{\vivekeq}[1]{\mbox{\tiny {\em #1}}}
\newcommand{\Tlife}{T_{\mbox{\tiny \em life}}}
\newcommand{\Ieff}{I_{\mbox{\tiny \em eff}}}
\newcommand{\Irise}{I_{\mbox{\tiny \em rise}}}
\newcommand{\Jpavg}{J_{\vivekeq{avg}}^+}
\newcommand{\Jnavg}{J_{\vivekeq{avg}}^-}
\newcommand{\Jbavg}{J_{\vivekeq{avg}}^{\vivekeq{blue}}}
\newcommand{\Jgavg}{J_{\vivekeq{avg}}^{\vivekeq{green}}}
\newcommand{\nuc}{t_{\mbox{\scriptsize \it nuc}}}
\newcommand{\nucs}{t_{\mbox{\scriptsize \it nuc--SI}}}
\newcommand{\nucf}{t_{\mbox{\scriptsize \it nuc--F}}}
\newcommand{\tlife}{t_{\mbox{\scriptsize \it life}}}
\newcommand{\Mx}{\mbox{M}_{\mbox{\scriptsize x}}}
\newcommand{\Mxp}{\mbox{M}_{\mbox{\scriptsize x+1}}}
\pagestyle{plain}
\renewcommand{\bibfont}{\tiny}
\usepackage{tikz}
\usetikzlibrary{shapes,arrows}
\renewcommand{\baselinestretch}{1.000}
%\selectcolormodel{gray}


==> tbl/table_lut.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
%\pm 0.76 \pm 2.74  \pm 2.21 \pm 2.69

\begin{table}[hbt]
\caption{Statistics of test designs}
\label{tbl:data}
\centering
%\resizebox{1.00\columnwidth}{!}{%
\begin{tabular}{@{}|c|c|c|@{}}
\hline

Method                 & \#nodes & \#Edges \\ \hline
%All disconnected nodes & 67.32 $\pm$ 0.76 \\ \hline
OTA            & 27 & 34 \\ \hline
R2R ladder            & 116 & 144 \\ \hline
FIR equalizer            & 640  & 1099 \\ \hline

\end{tabular}%
%}
\end{table}

